Geometric deep learning: going beyond Euclidean data

Many scientific fields study data with an underlying structure that is a non-Euclidean space. Some examples include social networks in computational social sciences, sensor networks in communications, functional networks in brain imaging, regulatory networks in genetics, and meshed surfaces in computer graphics. In many applications, such geometric data are large and complex (in the case of social networks, on the scale of billions), and are natural targets for machine learning techniques. In particular, we would like to use deep neural networks, which have recently proven to be powerful tools for a broad range of problems from computer vision, natural language processing, and audio analysis. However, these tools have been most successful on data with an underlying Euclidean or grid-like structure, and in cases where the invariances of these structures are built into networks used to model them. Geometric deep learning is an umbrella term for emerging techniques attempting to generalize (structured) deep neural models to non-Euclidean domains such as graphs and manifolds. The purpose of this paper is to overview different examples of geometric deep learning problems and present available solutions, key difficulties, applications, and future research directions in this nascent field.

==> abstract.tex <==
In recent years, increasingly more fields have to deal with data coming from non-Euclidean domains such as manifolds or graphs. For instance, in social networks, the characteristics of users can be modeled as signals on the vertices of the social graph \cite{lazer2009life}. Sensor networks are graph models of distributed interconnected sensors, whose readings are modelled as time-dependent signals on the vertices. In genetics, gene expression data are modeled as signals defined on the regulatory network \cite{davidson2002genomic}. 
%
In neuroscience, graph models are used to represent anatomical and functional structures of the brain. 
%
In computer graphics and vision, 3D objects are modeled as Riemannian manifolds (surfaces) endowed with properties such as color texture. Even more complex examples include networks of operators, e.g., functional correspondences \cite{ovsjanikov2012functional} or difference operators \cite{rustamov2013map} in a collection of 3D shapes, or orientations of overlapping cameras in multi-view vision (``structure from motion'') problems \cite{arie2012global}. Furthermore, modeling high-dimensional data with graphs is an increasingly popular trend in general data science, where graphs are used to describe the low-dimensional intrinsic structure of the data.


The complexity of geometric data and the availability of very large datasets (in the case of social networks, of the billion-scale) make it tempting and very desirable to resort to machine learning techniques. Yet, currently available learning methods have been developed primarily for Euclidean data and are not suitable for the non-Euclidean setting. 

The purpose of this paper is to overview the problems arising in relation to geometric deep learning and present solutions existing today for this class of problems, as well as key difficulties and future research directions.




==> bios.tex <==
\begin{IEEEbiographynophoto}{Michael M. Bronstein}
(PhD with distinction 2007, CS Technion, Israel) is an Associate Professor 
%in the Institute of Computational Science, Faculty of Informatics 
at the USI Lugano, Switzerland and Tel Aviv University, Israel. He also serves as a 
%Research Scientist and 
Principal Engineer at Intel Perceptual Computing. 
%He previously held visiting positions at the Technion and Stanford University. 
His main research interest is in theoretical and computational methods for geometric data analysis. He authored over 150 papers, the book {\em Numerical geometry of non-rigid shapes} (Springer 2008), and over 20 granted patents. He was awarded three ERC grants (Starting 2012, Proof of Concept 2016, and Consolidator 2016), Google Faculty Research award (2016), and Radcliffe fellowship (2017) at the Harvard Institute for Advanced Study, and Rudolf Diesel fellowship (2017) at TU Munich. He was invited as a Young Scientist to the World Economic Forum, an honor bestowed on forty worldÕs leading scientists under the age of forty. 
%
Michael is an ACM Distinguished Speaker, Associate editor of CVIU (2013-present), and Area Chair at ECCV 2016 and ICCV 2017.
%
In addition to academic work, Michael is actively involved in commercial technology development and consulting to start-up companies. 
%He is the holder of over 20 granted technological patents and over 30 patent applications. 
He was a co-founder and technology executive at Novafora (2005-2009) developing large-scale video analysis methods, and one of the chief technologists at Invision (2009-2012) developing low-cost 3D sensors. Following the multi-million acquisition of Invision by Intel in 2012, Michael has been one of the key developers of the Intel RealSense technology.
\end{IEEEbiographynophoto}


\begin{IEEEbiographynophoto}{Joan Bruna}
graduated from Universitat Polit{\`e}cnica de Catalunya (Barcelona, Spain) in both Mathematics and Electrical Engineering. He obtained an M.Sc. in applied mathematics from ENS Cachan (France). He then became a research engineer in an image processing startup, developing realtime video processing algorithms. He obtained his PhD in Applied Mathematics at Ecole Polytechnique (France), under the supervision of Prof. St{\'e}phane Mallat. He was a postdoctoral researcher at the Courant Institute, NYU, New York, and a postdoctoral fellow at Facebook AI Research. In 2015, he became Assistant Professor at UC Berkeley, Statistics Department, and starting Fall 2016 he joined the Courant Institute (NYU, New York) as Assistant Professor in Computer Science, Data Science and Mathematics (affiliated). 
%
His research interests include invariant Signal representations, high-dimensional statistics and Stochastic processes, Deep Learning, and its applications to signal processing.
\end{IEEEbiographynophoto}



\begin{IEEEbiographynophoto}{Yann LeCun} (PhD 1987, Universit{\`e} Pierre et Marie Curie) 
is Director of AI Research at Facebook and Silver Professor at NYU. 
%of Dara Science, Computer Science, Neural Science, and Electrical Engineering at New York University, affiliated with the NYU Center for Data Science, the Courant Institute of Mathematical Science, the Center for Neural Science, and the Electrical and Computer Engineering Department.
%He received the Electrical Engineer Diploma from Ecole Superieure d'Ingenieurs en Electrotechnique et Electronique (ESIEE), Paris in 1983, and a PhD in Computer Science from Universite Pierre et Marie Curie (Paris) in 1987. 
After a postdoc at the University of Toronto, he joined AT\&T Bell Labs in Holmdel in 1988, where he became head of the Image Processing Research Department. % at AT\&T Labs-Research in 1996, 
He joined NYU as a professor in 2003, after a brief period as a Fellow of the NEC Research Institute in Princeton. 
%From 2012 to 2014 he directed NYU's initiative in data science and became the founding director of the NYU Center for Data Science. He was named Director of AI Research at Facebook in late 2013 and retains a part-time position on the NYU faculty.
%His current interests include AI, machine learning, computer perception, mobile robotics, and computational neuroscience. He has published over 180 technical papers and book chapters on these topics as well as on neural networks, handwriting recognition, image processing and compression, and on dedicated circuits and architectures for computer perception. The character recognition technology he developed at Bell Labs is used by several banks around the world to read checks and was reading between 10 and 20\% of all the checks in the US in the early 2000s. His image compression technology, called DjVu, is used by hundreds of web sites and publishers and millions of users to access scanned documents on the Web. 
Since the late 80's, LeCun has been working on deep learning methods, particularly the convolutional network model, which is the basis of many products and services deployed by companies such as Facebook, Google, Microsoft, Baidu, IBM, NEC, AT\&T and others for image and video understanding, document recognition, human-computer interaction, and speech recognition. 
LeCun is a member of the US National Academy of Engineering and has been on the editorial board of IJCV, IEEE PAMI, and IEEE Trans. Neural Networks, was program chair of CVPR 2006 and chair of ICLR 2013 and 2014. He is on the science advisory board of Institute for Pure and Applied Mathematics, and has advised many large and small companies about machine learning technology, including several startups he co-founded. 
%He is the lead faculty at NYU for the Moore-Sloan Data Science Environment, a \$36M initiative in collaboration with UC Berkeley and University of Washington to develop data-driven methods in the sciences. 
He received the IEEE Neural Network Pioneer Award (2014), PAMI Distinguished Researcher award (2015), and Doctor Honoris Causa from IPN in Mexico City. 
\end{IEEEbiographynophoto}




\begin{IEEEbiographynophoto}{Arthur Szlam}
is a research scientist at Facebook AI Research. He received the PhD under Prof. Ronald Coifman at Yale University. Prior to joining Facebook, he was a postdoctoral fellow at the Institute for Mathematics and its Applications (IAM) at the University of Minnesota and the Institute for Pure and Applied Mathematics (IPAM) UCLA, and an assistant professor at City College of New York. He is a Sloan Foundation fellow. His research interests are in computational harmonic analysis, the relationships between smoothness, frequency, and scale on graphs and data clouds, and applications to signal processing and machine learning. 
\end{IEEEbiographynophoto}




\begin{IEEEbiographynophoto}{Pierre Vandergheynst}
(PhD in Mathematical Physics 1998, UCL, Belgium) 
is a Full Professor at the Swiss Federal Institute of Technology (EPFL), Switzerland. 
%received the M.S. degree in physics and the Ph.D. degree in mathematical physics from the UniversitŽ catholique de Louvain, Louvain-la-Neuve, Belgium, in 1995 and 1998, respectively. From 1998 to 2001, he was a Postdoctoral Researcher with the Signal Processing Laboratory, Swiss Federal Institute of Technology (EPFL), Lausanne, Switzerland. He was Assistant Professor at EPFL (2002-2007), where he is now a Full Professor and Vice Provost. 
%
His research focuses on harmonic analysis, sparse approximations and mathematical image processing with applications to higher dimensional, complex data processing. He was co-Editor-in-Chief of Signal Processing (2002-2006) and is Associate Editor of the IEEE Transactions on Signal Processing (2007-present). He has been on the Technical Committee of various conferences and was Co-General Chairman of the EUSIPCO 2008 conference. Pierre Vandergheynst is the author or co-author of more than 50 journal papers, one monograph and several book chapters. He is a laureate of the Apple ARTS award and of the 2010-2011 De Boelpaepe prize from the Royal Academy of Sciences of Belgium. Pierre is strongly involved in technology transfer: he co-founded two start-ups and holds numerous patents.
\end{IEEEbiographynophoto}



==> freqj.tex <==
\section{Spectral methods}
\label{sec:freq}

We have now finally got to our main goal, namely, constructing a generalization of the CNN architecture on non-Euclidean domains. %to graphs. 
%
We will start with the assumption that the domain on which we are working is fixed, and for the rest of this section will use the problem of classification of a signal on a fixed graph as the prototypical application.  

%\paragraph*{\bf Spectral CNN}

%As in section \ref{sec:noneucl}, 
%let $W$ be a  weighted graph with index set denoted by $\Omega$, and let $\boldsymbol{\Phi}$
% be the unitary matrix containing the 
% eigenvectors of the graph Laplacian $\boldsymbol{\Delta}$, ordered by eigenvalue.
%In Section \ref{sec:noneucl}, 
%\paragraph*{\bf Spectral approaches}
We have seen that convolutions are linear operators that commute 
 with the Laplacian operator. Therefore, 
given a weighted graph, a first route to generalize a convolutional architecture is by first
restricting our interest to linear operators that commute with the graph Laplacian. % \cite{bruna2013spectral}.
This property, in turn, implies operating on the spectrum of the 
graph weights, given by the eigenvectors of the graph Laplacian.

% m->p (input), n->q


{\bf{\em Spectral CNN (SCNN)}} \cite{bruna2013spectral}: Similarly to the convolutional layer~(\ref{eq:convlayer}) of a classical Euclidean CNN, Bruna et al. \cite{bruna2013spectral} define a {\em spectral convolutional layer} as 
%
%For simplicity, let us first describe a construction where each layer $k=1\dots K$ 
%transforms an input vector $f_k$ of size $|\Omega| \times N_{k-1}$ into an output $f_{k+1}$ 
%of dimensions $|\Omega| \times N_{k}$, that is, without spatial subsampling:
\begin{equation} 
\label{spectral_construction_eq}
\mathbf{g}_l =   \xi \left(  \sum_{l'=1}^{q} \boldsymbol{\Phi}_k \mathbf{W}_{l,l'} \boldsymbol{\Phi}_k^\top \mathbf{f}_{l'} \right),
%f_{k+1, l}  =   \rho \left( \boldsymbol{\Phi} \sum_{l'=1}^{N_{k-1}} W_{k,l,l'} \boldsymbol{\Phi}^T f_{k,l'} \right)~,~l=1\dots N_k~,
\end{equation}
%
where the $n\times p$ and $n\times q$ matrices $\mathbf{F} = (\mathbf{f}_1, \hdots, \mathbf{f}_p)$  and $\mathbf{G} = (\mathbf{g}_1, \hdots, \mathbf{g}_q)$ represent the $p$- and $q$-dimensional input and output signals on the vertices of the graph, respectively (we use $n = |\mathcal{V}|$ to denote the number of vertices in the graph), 
$\mathbf{W}_{l,l'}$ is a $k\times k$ diagonal matrix of spectral multipliers representing a filter in the frequency domain, and $\xi$ is a nonlinearity applied on the vertex-wise function values. 
%
Using only the first $k$ eigenvectors in~(\ref{spectral_construction_eq}) sets a cutoff frequency which depends on the intrinsic regularity of the graph and also the sample size. Typically,  $k \ll n$, since only the first Laplacian eigenvectors describing the smooth structure of the graph are useful in practice. 

%
%Often, only the first $d$ eigenvectors of the Laplacian are useful in practice, which  
%carry the smooth geometry of the graph.  $\boldsymbol{\Phi}$ by
%$\boldsymbol{\Phi}_d$, obtained by keeping the first $d$ columns of $\boldsymbol{\Phi}$.

If the graph has an underlying group invariance, such a construction can discover it. In particular, 
standard CNNs can be redefined from the spectral domain (see insert IN5). %; see \ref{sec:rediscover}. 
However, in many cases the graph does not 
have a group structure, or the group structure does not commute with the Laplacian, 
and so we cannot think of each filter as passing a template across $\mathcal{V}$ and recording the correlation 
of the template with that location. 




%\paragraph*{\bf Limitations of Spectral CNNs}

We should stress that a fundamental limitation of the spectral construction is its limitation to a single domain. 
%
The reason is that spectral filter coefficients~(\ref{spectral_construction_eq}) are {\em basis dependent}. It implies that if we learn a filter w.r.t. basis $\boldsymbol{\Phi}_k$ on one domain, and then try to apply it on another domain with another basis $\boldsymbol{\Psi}_k$, the result could be very different (see Figure~2 and insert IN6). 
%~\ref{fig:blobs} and insert IN6). 
%
%Consequently, spectral CNN can be considered as method for learning on a graph, rather than on multiple graphs. 
%
It is possible to construct compatible orthogonal bases across different domains resorting to a joint diagonalization procedure \cite{kovnatsky2013coupled,eynard2015multimodal}. However, such a construction requires the knowledge of some correspondence between the domains. In applications such as social network analysis, for example, where dealing with two time instances of a social graph in which new vertices and edges have been added, such a correspondence can be easily computed and is therefore a reasonable assumption. 
%
Conversely, in computer graphics applications, finding correspondence between shapes is in itself a very hard problem, so assuming known correspondence between the domains is a rather unreasonable assumption. 
%
%In the next section, we will see a different generalization of the convolution that allows applying CNN-type models across different domains. 


\begin{figure}[h!]
\centering
\begin{overpic}
[width=1\linewidth]{dots.pdf}
%
\put(0,-4){\small Domain}
\put(0,-9){\small Basis}
\put(0,-14){\small Signal}
%
\put(18,-4){\small $\mathcal{X}$}
\put(18,-9){\small $\boldsymbol{\Phi}$ }%$\{ \phi \}_{i\geq 0}$}
\put(18,-14){\small $\mathbf{f}$}
%
\put(58.5,-4){\small $\mathcal{X}$}
\put(58.5,-9){\small $\boldsymbol{\Phi}$ }%$\{ \phi \}_{i\geq 0}$}
\put(54.5,-14){\small $\boldsymbol{\Phi} \mathbf{W} \boldsymbol{\Phi}^\top\mathbf{f}$}%$\sum_{i\geq 0} \hat{w}_i \langle f,\phi_i \rangle_{L^2(\mathcal{X})} \phi_i$}
%
\put(90,-4){\small $\mathcal{Y}$}
\put(90,-9){\small $\boldsymbol{\Psi}$} %$\{ \psi \}_{i\geq 0}$}
\put(85,-14){\small $\boldsymbol{\Psi} \mathbf{W} \boldsymbol{\Psi}^\top\mathbf{f}$} %$\{ \psi \}_{i\geq 0}$}
\end{overpic}
\vspace{10mm}
\label{fig:blobs}
\caption{
\small A toy example illustrating the difficulty of generalizing spectral filtering across non-Euclidean domains. 
Left: a function defined on a manifold (function values are represented by color); middle: result of the application of an edge-detection filter in the frequency domain; right: the same filter applied on the same function but on a different (nearly-isometric) domain produces a completely different result. The reason for this behavior is that the Fourier basis is domain-dependent, and the filter coefficients learnt on one domain cannot be applied to another one in a straightforward manner.
}
\end{figure}





%Number of parameters
Assuming that $k = O(n)$ eigenvectors of the Laplacian are kept, 
a convolutional layer~(\ref{spectral_construction_eq}) requires 
$p q k = O(n)$ parameters to train. 
We will see next how the global and local 
regularity of the graph can be combined to produce layers with constant number of
parameters (i.e., such that the number of learnable parameters per layer does not depend upon 
the size of the input), which is the case in classical Euclidean CNNs. 

%Another important property that relates classical Euclidean CNN with the 
%spectral domain construction is the downsampling or pooling operation. 

The non-Euclidean analogy of pooling is {\em graph coarsening}, in which only a fraction $\alpha < 1$ of the graph vertices is retained. 
%
The eigenvectors of graph Laplacians at two different resolutions are related by the following
multigrid property: Let $\boldsymbol{\Phi}$, $\tilde{\boldsymbol{\Phi}}$ denote the $n \times n$ and $\alpha n \times \alpha n$ matrices of Laplacian eigenvectors of the original and the coarsened graph, respectively.  
%denote the eigenvectors of the original graph Laplacian and the coarse graph Laplacian 
%respectively (where we kept a fraction $\alpha$ of the nodes), then 
Then, 
\begin{equation}
\tilde{\boldsymbol{\Phi}} \approx \mathbf{P} \boldsymbol{\Phi} \left( 
\begin{array}{c} 
\mathbf{I}_{\alpha n} \\
\mathbf{0}
\end{array}
\right), 
\end{equation}
where $\mathbf{P}$ is a $\alpha n \times n$ binary matrix whose $i$th row encodes the position of the $i$th vertex of the coarse graph on the original graph. 
%
It follows that strided convolutions can be generalized using the spectral construction by keeping
only the low-frequency components of the spectrum.
This property also allows us to interpret (via interpolation) 
the local filters at deeper layers in the spatial construction to be low frequency.  
However, since in~(\ref{spectral_construction_eq}) the non-linearity is applied in the spatial domain, 
in practice one has to recompute the graph Laplacian eigenvectors at each resolution and apply them directly 
after each pooling step.


%The spectral construction can suffer from the fact that most graphs have meaningful eigenvectors 
%only for the very top of the spectrum. 
%Even when the individual high frequency eigenvectors are not 
%meaningful, a cohort of high frequency eigenvectors may contain meaningful information.  However 
%this construction may not be able to access this information because it is nearly diagonal at the highest frequencies.  
The spectral construction (\ref{spectral_construction_eq}) assigns a degree of freedom for each 
eigenvector of the graph Laplacian. In most graphs, individual high-frequency eigenvectors become highly unstable.  
%as one accesses smaller eigenvalues, which are associated with higher frequency information. 
However, 
similarly as the wavelet construction in Euclidean domains, by appropriately grouping high frequency 
eigenvectors in each octave one can recover meaningful and stable information. As we shall see 
next, this principle also entails better learning complexity. 

 %{\color{red}MB: This is not clear to me- Joan, can you explain what is meant here?}




% it is not obvious how to do either the forwardprop or the backprop efficiently while applying the nonlinearity 
%on the space side, as we have to make the expensive multiplications by $V$ and $V^T$; and it is not obvious 
%how to do standard nonlinearities on the spectral side. However, see \ref{sec:multigrid}.  
% 
%Why is the previous spectral construction not always good? 
%Stability with respect to noise / sampling. Only the regular part of the spectrum is in practice stable. 
%High frequencies are important for recognition and are not efficiently captured with 
%the Laplacian eigenmaps.
 
 \myframedtext*[\linewidth]{
\vspace{-5mm}
\begin{multicols}{2}
 \paragraph*{\bf [IN5] Rediscovering standard CNNs using correlation kernels}
 \label{sec:rediscover}
 In situations where the graph is constructed from the data, a straightforward choice of the edge weights~(\ref{eq:graph_lap}) of the graph 
is the covariance of the data.  
%
Let $\mathbf{F}$ denote the input data distribution and %, where each row represents a data point, and denote by 
\begin{equation}
\boldsymbol{\Sigma} = \E (\mathbf{F} - \E \mathbf{F}) (\mathbf{F} - \E \mathbf{F})^\top
\end{equation}
be the data covariance matrix. If each point has the same variance $\sigma_{ii} = \sigma^2$, 
%%
%Let $\mathbf{F}=(f_k)_k$ be the input data distribution, with $f_k \in \mathbb{R}^n$.
%If each coordinate $j=1\dots n$ has the same variance,  
%$$\sigma^2_j = \E\left( | f(j) -  \E(f(j))|^2\right)~,$$
then diagonal operators on the Laplacian simply scale the principal components of $\mathbf{F}$.  \\
%
In natural images, since their distribution is approximately stationary, 
%its covariance operator 
%$$\Sigma(j,j) = \E\left( (f(j) -  \E(f(j)))(f(j') -  \E(f(j')))\right) $$
%satisfies $\Sigma(j,j') = \Sigma(j-j')$, hence it is 
the covariance matrix has a circulant structure $\sigma_{ij} \approx \sigma_{i-j}$ and is thus 
diagonalized by the standard Discrete Cosine Transform (DCT) basis. 
%
It follows that the principal 
components of $\mathbf{F}$ roughly correspond to the DCT basis vectors %Discrete Cosine Transform basis, 
ordered by frequency. 
%
 Moreover, natural images exhibit a power spectrum $\E |\widehat{f}(\omega)|^2 \sim |\omega|^{-2} $, 
since nearby pixels are more correlated than far away pixels \cite{simoncelli2001natural}.
It results that principal components of the covariance are essentially ordered from
low to high frequencies, which is consistent with the standard group structure of the 
Fourier basis.
When applied to natural images represented as graphs with weights defined by the covariance, the spectral CNN construction   
recovers the standard CNN, 
 without any prior knowledge %. This property was also studied in 
 \cite{roux2008learning}. 
 Indeed, the linear operators $\boldsymbol{\Phi} \mathbf{W}_{l,l'} \boldsymbol{\Phi}^\top$ in~(\ref{spectral_construction_eq}) 
 are by the previous argument diagonal in the Fourier basis, hence translation invariant, 
 hence classical convolutions. 
 %
 Furthermore, Section \ref{sec:freq} explains how spatial 
 subsampling can also be obtained via dropping the last part of the spectrum of the Laplacian, 
 leading to pooling, and ultimately to standard CNNs.
%
\begin{center}\vspace{3mm}
\begin{overpic}
%\input{fig1.tex}
[width=0.45\linewidth]{emb_x_rbf.png}
\end{overpic}\hspace{5mm}
\begin{overpic}
%\input{fig2.tex}
[width=0.45\linewidth]{emb_y_rbf.png}
\end{overpic}
\end{center}\vspace{0mm}
{\small {\bf [FIG5a]} Two-dimensional embedding of pixels in $16\times 16$ image patches using a Euclidean RBF kernel. 
The RBF kernel is constructed as in (\ref{eq:graph_lap}), by using the covariance 
$\sigma_{ij}$ as Euclidean distance between two features. The pixels are embedded in a 2D space using the first two eigenvectors of the resulting graph Laplacian. The colors in the left and right figure represent the horizontal and vertical coordinates of the pixels, respectively. 
The spatial arrangement of pixels is roughly recovered from correlation measurements.
}
  \end{multicols}
}



%\paragraph*{\bf 
{\bf{\em Spectral CNN with smooth spectral multipliers}} \cite{bruna2013spectral,henaff2015deep}:
%Learning with smooth spectral multipliers}
%\label{smoothspect}
%
In order to reduce the risk of overfitting, it is important to adapt the learning 
complexity to reduce the number of free parameters of the model. 
On Euclidean domains, this is achieved by learning convolutional kernels with small spatial support,  which enables the model to learn a number of parameters independent of the input size. 
%
In order to achieve a similar learning complexity in the spectral domain, it is thus necessary to restrict the class of spectral multipliers to those corresponding to localized filters. 

For that purpose, we have to express spatial localization of filters in the frequency domain. 
%
In the Euclidean case, smoothness in the frequency domain corresponds to  spatial decay, since
%$$\left| \frac{\partial^k \hat{f}(\omega)}{\partial \omega^k} \right| \leq C \int^{+\infty}_{-\infty} |x|^k |f(x)| dx.$$
\begin{equation}
\int_{-\infty}^{+\infty} |x|^{2k} |f(x)|^2 dx = \int_{-\infty}^{+\infty} \left| \frac{\partial^k \hat{f}(\omega)}{\partial \omega^k} \right|^2 d\omega,
\end{equation}
by virtue of the Parseval Identity.
%where $\hat{f}(\omega)$ is the Fourier transform of $f$.
%
% In the standard grid, we do not need a parameter for each 
% frequency because the filters 
% are compactly supported in space, but in (\ref{spectral_construction_eq}), 
% each filter requires one parameter for each eigenvector on which it acts. 
% Even if the filters were compactly supported in space in this construction, 
% we still would not get less than $O(N)$ parameters per filter because the spatial 
% response would be different at each location.  
 %
% One possibility for getting around this is to generalize the duality of the grid.  
% On the Euclidian grid, the decay of a function in the spatial domain is translated 
% into smoothness in the Fourier domain, and viceversa. 
%It results that a function $x$ which is spatially localized 
%  has a smooth frequency response $\hat{x} = V^T x$. 
%In that case, the eigenvectors of the Laplacian can be thought of as being arranged on a grid 
%isomorphic to the original spatial grid.
%
This suggests that, in order to learn a layer in which features will be not only 
shared across locations but also well localized in the original domain,
one can learn spectral multipliers which are smooth. 
%
Smoothness can be prescribed by learning only a subsampled set
of frequency multipliers and using an interpolation kernel 
to obtain the rest, such as cubic splines.


However, the notion of smoothness also requires some geometry in the spectral domain.  
%
In the Euclidean setting, such a geometry naturally arises from the notion of frequency; for example, in the plane, the similarity between two Fourier atoms $e^{i \boldsymbol{\omega}^\top \mathbf{x}}$ and $e^{i \boldsymbol{\omega'}^\top \mathbf{x}}$
 can be quantified by the distance $\| \boldsymbol{\omega} - \boldsymbol{\omega'}\|$, where $\mathbf{x}$ denotes the two-dimensional planar coordinates, and $\boldsymbol{\omega}$ is the two-dimensional frequency vector. 
 %
On graphs, such a relation 
% but this cannot be directly generalized to other graphs. 
can be defined by means of a dual graph %$\widetilde{W}=(\tilde{w}_{i,j})$ 
with weights $\tilde{w}_{ij}$ encoding the similarity between two eigenvectors $\phi_i$ and $\phi_j$.


A particularly simple choice consists in choosing a 
one-dimensional arrangement, obtained by ordering the eigenvectors according
to their eigenvalues. \footnote{
In the mentioned 2D example, this would correspond to ordering the Fourier basis function according to the sum of the corresponding  frequencies $\omega_1 + \omega_2$. 
Although numerical results on simple low-dimensional graphs show that the 1D arrangement 
given by the spectrum of the Laplacian is efficient at creating spatially localized filters \cite{bruna2013spectral}, an open fundamental question is how to define a dual graph on the eigenvectors of the Laplacian in which smoothness (obtained by 
applying the diffusion operator) corresponds to localization in the original graph. 
}
In this setting, 
the spectral multipliers are parametrized as %diagonal of each filter $\mathbf{W}_{l,l'}$ (of size at most $|\Omega|)$ is parametrized by
% 
\begin{equation}
\label{eq:bspline}
\mbox{diag}(\mathbf{W}_{l,l'}) = \mathbf{B} \boldsymbol{\alpha}_{l,l'}, 
\end{equation}
%
where $\mathbf{B} = (b_{ij}) = (\beta_j(\lambda_i))$ is a $k \times q$ 
fixed interpolation kernel (e.g., $\beta_j(\lambda)$ can be cubic splines) and 
$\boldsymbol{\alpha}$ is a vector of $q$ interpolation coefficients. 
In order to obtain filters with constant spatial support (i.e., independent of the input size $n$), 
one should choose a sampling step $\gamma \sim n$ in the spectral domain, which 
results in a constant number $n \gamma^{-1} = \mathcal{O}(1)$ of coefficients $\boldsymbol{\alpha}_{l,l'}$ per filter.
\editJB{
Therefore, by combining spectral layers with graph coarsening, this model has  
$\mathcal{O}( \log n)$ total trainable parameters for inputs of size $n$, thus recovering the same 
learning complexity as CNNs on Euclidean grids. }

Even with such a parametrization of the filters, the spectral CNN~(\ref{spectral_construction_eq}) entails a high computational complexity of performing 
forward and backward passes, since they require an expensive step of matrix multiplication  by $\boldsymbol{\Phi}_k$ and $\boldsymbol{\Phi}_k^\top$. While on Euclidean domains such a multiplication can be efficiently carried in $\mathcal{O}(n\log n)$ operations using FFT-type algorithms, for general graphs such algorithms do not exist and the complexity is $\mathcal{O}(n^2)$.
%
We will see next %in Section \ref{sec:spat_freq} the following 
how to alleviate this cost by avoiding explicit computation of the Laplacian eigenvectors. 

%A possible algorithmic strategy is to consider an input distribution $X=(x_k)_k$ consisting on spatially localized 
%signals and to construct a dual graph $\widehat{W}$ by measuring the similarity of 
%in the spectral domain: $\widehat{X}= V^T X$. 
%The similarity could be measured for instance
%with $E( ( |\hat{x}| -E(|\hat{x})|))^T( |\hat{x}| -E(|\hat{x}|))$.



%\paragraph*{\bf Spectrum-free computation}

%Chebyshev polynomials \cite{defferrard2016convolutional}


\section{Spectrum-free methods}
\label{sec:freq}


\editMB{
A polynomial of the Laplacian acts as a polynomial on the eigenvalues.   
Thus, instead of explicitly operating in the frequency domain with spectral multipliers as in equation~\eqref{eq:bspline}, it is possible to represent the filters 
%Another convenient parametric way of representing the convolution filters is 
via a polynomial expansion:}
\begin{eqnarray}
\label{eq:poly_filter}
	g_{\boldsymbol{\alpha}}(\boldsymbol{\Delta}) &=& \boldsymbol{\Phi} g_{\boldsymbol{\alpha}}(\boldsymbol{\Lambda}) \boldsymbol{\Phi}^\top, %\\
%	%
%	g_{\boldsymbol{\alpha}}(\boldsymbol{\Lambda}) &=& 
%	\left(
%	\begin{array}{ccc} 
%	g_{\boldsymbol{\alpha}}(\lambda_1) &&\\
%	&\cdots&\\
%	&&	g_{\boldsymbol{\alpha}}(\lambda_{n})
%\end{array}
%	\right)
\end{eqnarray}
%
corresponding to %~\cite{defferrard2016convolutional}. 
%
\begin{equation} \label{eq:filt_poly}
	g_{\boldsymbol{\alpha}}(\lambda) = \sum_{j=0}^{r-1} \alpha_j \lambda^j.
\end{equation}
%
Here $\boldsymbol{\alpha}$ is the $r$-dimensional vector of polynomial coefficients, and $g_{\boldsymbol{\alpha}}(\boldsymbol{\Lambda}) = \mathrm{diag}( g_{\boldsymbol{\alpha}}(\lambda_1), \hdots, g_{\boldsymbol{\alpha}}(\lambda_n) )$,  
resulting in filter matrices $\mathbf{W}_{l,l'} = g_{\boldsymbol{\alpha}_{l,l'}}(\boldsymbol{\Lambda})$ whose entries have an explicit form in terms of the eigenvalues.  

 
%
%In this case, the filter matrix $W_{k,l,l'}$ is a diagonal matrix whose entries have an explicit form in terms of the eigenvalues. Ignoring the filter index for the sake of clarity, we write $W_{l,l} = g_\theta(\lambda_l)$, where~:
%\begin{equation} \label{eq:filt_poly}
%	g_\theta(\Lambda) = \sum_{j=0}^{J-1} \theta_j \Lambda^j,
%\end{equation}
%and the parameter $\theta \in \mathbb{R}^J$ is a vector of polynomial coefficients. 

An important property of this representation is that it automatically yields localized filters, for the following reason.  
Since the Laplacian is a local operator (working on 1-hop neighborhoods), the action of its $j$th power is constrained to $j$-hops. Since the filter is a linear combination of powers of the Laplacian, overall  %$g_{\boldsymbol{\alpha}}(\boldsymbol{\Delta})$ 
(\ref{eq:filt_poly}) behaves like a diffusion operator limited to $r$-hops around each vertex. 

%Indeed, applying the spectral theorem, we can write $V W V^T = g_\theta(L)$ and we observe that filtering is obtained by applying a polynomial of the Laplacian operator. Such filters behave like diffusion operators, whose action is constrained to $J$-hop neighbourhoods. 

{\bf{\em Graph CNN (GCNN) a.k.a. ChebNet}} \cite{defferrard2016convolutional}: Defferrard et al. used 
%$g_{\boldsymbol{\alpha}}(\lambda)$ as a polynomial that can be computed recursively.  
%%Besides their ease of interpretation, polynomial filters can also be applied very efficiently if one chooses
%$g_{\boldsymbol{\alpha}}(\lambda)$ as a polynomial that can be computed recursively. For instance, the 
Chebyshev polynomial %$T_j(\lambda)$ of order $j$ 
generated by the recurrence relation 
\begin{eqnarray}
\label{eq:cheby}
T_j(\lambda) &=& 2\lambda T_{j-1}(\lambda) - T_{j-2}(\lambda);\\ 
T_0(\lambda) &=&1; \nonumber \\
T_1(\lambda) &=& \nonumber \lambda. 
\end{eqnarray}
A filter can thus be parameterized uniquely via an
 expansion of order $r-1$ such that
\begin{eqnarray} \label{eq:filt_cheby}
	g_{\boldsymbol{\alpha}}(\tilde{\boldsymbol{\Delta}}) &=& \sum_{j=0}^{r-1} \alpha_j  \boldsymbol{\Phi} T_j(\tilde{\boldsymbol{\Lambda}})\boldsymbol{\Phi}^\top \\
	&=& \sum_{j=0}^{r-1} \alpha_j T_j(\tilde{\boldsymbol{\Delta}}),  \nonumber
\end{eqnarray}
%where the parameter $\theta \in \mathbb{R}^J$ is a vector of Chebyshev coefficients and
%$T_j(\tilde{\Lambda}) \in \mathbb{R}^{n \times n}$ is the Chebyshev polynomial of order
%$j$ evaluated at 
where $\tilde{\boldsymbol{\Delta}} = 2 \lambda_{n}^{-1}\boldsymbol{\Delta}  - \mathbf{I}$ and $\tilde{\boldsymbol{\Lambda}} = 2 \lambda_{n}^{-1} \boldsymbol{\Lambda}  - \mathbf{I}$ denotes a rescaling of the Laplacian mapping its eigenvalues from the interval $[0, \lambda_{n}]$ to $[-1,1]$ (necessary since the Chebyshev polynomials form an orthonormal basis in $[-1,1]$).

%Filtering a signal $\mathbf{f}$ can now be written as 
%\begin{equation}
%g_{\boldsymbol{\alpha}}(\boldsymbol{\Delta}) \mathbf{f}
%= \sum_{j=0}^{r-1} \alpha_j T_j(\tilde{\boldsymbol{\Delta}}) \mathbf{f}, 
%\end{equation}
%where $\tilde{\boldsymbol{\Delta}} = 2 \lambda_{n}^{-1}\boldsymbol{\Delta}  - \mathbf{I}$ is the rescaled Laplacian. 
%$T_j(\tilde{L}) \in \mathbb{R}^{n
%\times n}$ is the Chebyshev polynomial of order $j$ evaluated at the re-scaled
%Laplacian $\tilde{L} = 2 L / \lambda_{max} - I_n$. %Note that the spectrum of the
%normalized Laplacian is bounded by $2$ \cite{book:Chung97Spectral}, such that
%the scaling can simply be $\tilde{L} = L - I_n$. 
Denoting $\bar{\mathbf{f}}^{(j)} =
T_j(\tilde{\boldsymbol{\Delta}})\mathbf{f}$, we can use the recurrence relation~(\ref{eq:cheby}) to compute
$\bar{\mathbf{f}}^{(j)} = 2\tilde{\boldsymbol{\Delta}} \bar{\mathbf{f}}^{(j-1)} - \bar{\mathbf{f}}^{(j-2)}$ with $\bar{\mathbf{f}}^{(0)} = \mathbf{f}$ and
$\bar{\mathbf{f}}^{(1)} = \tilde{\boldsymbol{\Delta}}\mathbf{f}$. The computational complexity of this procedure is therefore $\mathcal{O}(rn)$ operations and does not require an explicit computation of the Laplacian eigenvectors.
%\paragraph*{\bf Spectrum-free computation}
%
%Chebyshev polynomials \cite{defferrard2016convolutional}



{\bf{\em Graph Convolutional Network (GCN)}} \cite{welling2016}: Kipf and Welling simplified this  construction by further assuming $r=2$ and $\lambda_n \approx 2$, resulting in filters of the form
\begin{eqnarray}
g_{\boldsymbol{\alpha}}( \mathbf{f} ) &=& \alpha_0 \mathbf{f} + \alpha_1 (\boldsymbol{\Delta} - \mathbf{I}) \mathbf{f}   \nonumber \\
&=& \alpha_0 \mathbf{f} - \alpha_1 \mathbf{D}^{-1/2} \mathbf{W} \mathbf{D}^{-1/2} \mathbf{f}. 
\end{eqnarray}
%
Further constraining $\alpha = \alpha_0 = -\alpha_1$, one obtains filters represented by a single parameter, 
\begin{eqnarray}
g_\alpha( \mathbf{f} ) &=& \alpha ( \mathbf{I} + \mathbf{D}^{-1/2} \mathbf{W} \mathbf{D}^{-1/2}) \mathbf{f}. 
\end{eqnarray}
%
Since the eigenvalues of $\mathbf{I} + \mathbf{D}^{-1/2} \mathbf{W} \mathbf{D}^{-1/2}$ are now in the range $[0,2]$, repeated application of such a filter can result in numerical instability. This can be remedied by a renormalization
%
\begin{eqnarray}
\label{eq:welling}
g_\alpha( \mathbf{f} ) &=& \alpha \tilde{\mathbf{D}}^{-1/2} \tilde{\mathbf{W}} \tilde{\mathbf{D}}^{-1/2} \mathbf{f}, 
\end{eqnarray}
%
where $\tilde{\mathbf{W}} = \mathbf{W} + \mathbf{I}$ and $\tilde{\mathbf{D}} = \mathrm{diag}(\sum_{j \neq i} \tilde{w}_{ij})$. 

\editADS{
Note that though we arrived at the constructions of ChebNet and GCN starting in the spectral domain, they boil down to applying simple filters acting on the $r$- or 1-hop neighborhood of the graph in the spatial domain.   We consider these constructions to be examples of the more general Graph Neural Network (GNN) framework:}
%We can thus consider these as spatial-domain methods, which are discussed in the following section. 
%Furthermore, GCN can be formulated as an instance of the Graph Neural Network (GNN) model described in the next section.  
%The more general ChebNet can also be considered a spatial-domain method with $r$-hop spatial filters. 
 
%Note that this also can be considered an example of the GNN construction discussed in Section \ref{sec:spat} and Equation \eqref{eq:gnn}






{\bf{\em Graph Neural Network (GNN)}} \cite{GNN}: 
%Many of the spatial-domain methods described above require notions of charts and local orientations as a ``filter'' needs to be matched against a neighborhood.  
%The spatial-domain methods above use some notion of local Euclidean structure to define filtering operations. 
Graph Neural Networks generalize the notion of applying the filtering operations directly on the graph via the graph weights.
%
%A more general spatial construction on graphs has been proposed \cite{gori2005new,GNN} and has been simplified in \cite{GGSNN,comnets}.  
\editJB{
Similarly as Euclidean CNNs learn generic filters as linear combinations of localized, oriented bandpass and lowpass filters, a Graph Neural Network learns
at each layer a generic linear combination of graph low-pass and high-pass operators. These are given respectively by $f \mapsto \mathbf{W}f$ and $f \mapsto \mathbf{\Delta} f$, 
and are generated by the degree matrix $\mathbf{D}$ and the diffusion matrix $\mathbf{W}$.
Given a $p$-dimensional input signal on the vertices of the graph, represented by the $n\times p$ matrix $\mathbf{F}$, %, the application of the Laplacian is an intrinsic operation that can be broken down into $\mathbf{W}\mathbf{F}$ and $\mathbf{D}\mathbf{F}$. 
%
%we have so far 
%considered two fundamental intrinsic linear operators:
%$$(\mathbf{D}\mathbf{f})_i = \left( \sum_{j \neq i} w_{ij}\right) \mathbf{f}_i~,\text{and}~(\mathbf{W}\mathbf{f})_i = \sum_{j \neq i} w_{ij}  \mathbf{f}_j~.$$

the GNN considers a generic point-wise nonlinearity $\eta_{\boldsymbol{\theta}}: \R^p \times \R^p \to \R^q$, 
parametrized by trainable parameters $\boldsymbol{\theta}$, that is applied to all nodes of the graph. 
\begin{equation}
\label{eq:gnn}
\mathbf{g}_i = \eta_{\boldsymbol{\theta}} \left( (\mathbf{W}\mathbf{f})_i, (\mathbf{D}\mathbf{f})_i \right).
\end{equation}
In particular, choosing $\eta( \mathbf{a},\mathbf{b}) = \mathbf{b} - \mathbf{b}$ one recovers the Laplacian operator $\mathbf{\Delta}\mathbf{f}$, but more general, nonlinear choices for $\eta$ yield trainable, task-specific diffusion operators.}  
Similarly as with a CNN architecture, one can stack the resulting GNN layers $\mathbf{g} = C_{\boldsymbol{\theta}}(\mathbf{f})$ and interleave them with graph pooling operators.
Chebyshev polynomials  $T_r(\mathbf{\Delta})$  can be obtained with $r$ layers of (\ref{eq:gnn}), making it possible, in principle, to consider ChebNet and GCN as particular instances of the GNN framework. 
%Some of the previous constructions can be cast as special cases of~(\ref{eq:gnn}). 

\editADS{
Historically, a version of GNN was
the first formulation of deep learning on graphs, proposed
in \cite{gori2005new,GNN}.  These works optimized over the parameterized steady state of some diffusion
process (or random walk) on the graph.  This can be interpreted as in equation \eqref{eq:gnn}, but using a large number of layers where each $C_{\boldsymbol{\theta}}$ is identical, as the forwards through the $C_{\boldsymbol{\theta}}$ approximate the steady state.   Recent works \cite{GGSNN,comnets,physical_dynamics,interaction_networks} relax the requirements of approaching the steady state or using repeated applications of the same $C_{\boldsymbol{\theta}}$.  




%The construction uses parameterized functions $f^k$ corresponding to the $k$th layer of the network; these input a vector $h^{k-1}_i$ associated to vertex $i$ in the graph, and a vector $c^{k-1}_i$ associated to vertex $i$ representing the communication of the neighbors of $i$ to $i$.   The $h$ and $c$ are updated via   
%\begin{eqnarray}
%h^{k+1}_i &=& f^k(h^{k}_j, c^{k}_j)  \\ 
%c^{k+1}_i &=& \frac{1}{s_i}\sum_{j}  w_{ij} h^{k+1}_{j}.
%\label{eq:gnn}
%\end{eqnarray}
%Note that the computation does not need the graph to defined until the network is to be evaluated.   Thus the learnable functions $f^k$ are decoupled from the graph structure, and are not fixed to use one specific graph.  This is the crux of the models flexibility: the model eats a graph, and outputs vectors on the nodes.   

Because the communication at each layer is local to a vertex neighborhood, one may worry that it would take many layers to get information from one part of the graph to another, requiring multiple hops (indeed, this was one of the reasons for the use of the steady state in \cite{GNN}). 
 However, for many applications, it is not necessary for information to completely traverse the graph.   Furthermore, note that the graphs at each layer of the network need not be the same.  Thus we can replace the original neighborhood structure with one's favorite multi-scale coarsening of the input graph, and operate on that to obtain the same flow of information as with the convolutional nets above (or rather more like a ``locally connected network'' \cite{coates2011selecting}).  This also allows producing a single output for the whole graph (for ``translation-invariant" tasks), rather than a per-vertex output, by connecting each to a special output node.  Alternatively, one can allow $\eta$ to use not only $\mathbf{W}\mathbf{f}$ and $\mathbf{\Delta}\mathbf{f}$ at each node, but also $\mathbf{W}^s \mathbf{f}$ for several diffusion scales $s>1$, (as in \cite{defferrard2016convolutional}), giving the GNN the ability to learn algorithms such as the power method, and more directly accessing spectral properties of the graph.
 
The GNN model can be further generalized to replicate other operators on graphs. For instance, 
the point-wise nonlinearity $\eta$ can depend on the vertex type, allowing extremely rich  architectures \cite{GGSNN,comnets,physical_dynamics,interaction_networks}. 
 
}

%\editMB{It thus allows formulating spectrum-free methods such as GCN as instances of GNN.}




==> intro.tex <==
\section{Introduction}
\label{sec:intro}

``Deep learning'' refers to learning complicated concepts by means of building them out of simpler ones in a hierarchical or Òmulti-layerÓ manner \cite{Goodfellow-et-al-2016-Book}. Artificial neural networks are popular realizations of such deep multi-layer hierarchies inspired by the signal processing in the human brain. In the past few years, the growing computational power of modern GPU-based computers, availability of large training datasets, and efficient stochastic optimization methods allowed creating and effectively training complex network models with many layers and degrees of freedom \cite{lecun2015deep}. This allowed deep neural networks to achieve a qualitative breakthrough in performance on a wide variety of tasks, from speech recognition \cite{mikolov2011strategies,hinton2012deep} and machine translation \cite{sutskever2014sequence} to image analysis and computer vision \cite{lecun2010convolutional,cirecsan2011committee,krizhevsky2012imagenet,farabet2013learning,taigman2014deepface,simonyan2014very,he2015deep}, igniting the renaissance of the field. Nowadays, deep learning methods are already widely used in commercial applications, including Siri speech recognition in Apple iPhone, Google text translation, and Mobileye vision-based technology for autonomously driving cars. 
%Several novel fields of applications of deep learning, such as Deep Genomics \cite{alipanahi2015predicting}, have the promise to become groundbreaking.


Among the key reasons for the success of deep neural networks are important assumptions on the statistical properties of the data, namely stationarity and compositionality through local statistics, which are present in natural images, video, and speech \cite{simoncelli2001natural, field1989statistics}, which were initially developed to model aspects of the visual cortex \cite{hopfield1982neural,olshausen1997sparse}. These statistical properties have been related to physics %via the renormalization group 
\cite{mehta2014exact} and formalized in specific classes of convolutional neural networks (CNNs) \cite{mallat2012group,bruna2013invariant,tygert2016mathematical}.
%{\color{blue} JB: updated with references}.
%{\color{green} ADS: lots more references in this seciton, no? specifically towards  images: http://www.naturalimagestatistics.net/, http://redwood.psych.cornell.edu/papers/field1989.pdf, and the Olshausen and Field sparse coding paper.    For compositionality and pooling etc, the renormalization paper http://arxiv.org/abs/1410.3831 and some scattering papers, and maybe Mark's version too }

 From the geometric perspective, one can think of images as functions on the Euclidean space (plane), sampled on a grid. In this setting, stationarity is owed to shift-invariance, locality is due to the local connectivity, and compositionality stems from the multi-resolution structure of the grid. These properties are exploited by convolutional architectures \cite{lecun1989backpropagation}, which are built of alternating convolutional and downsampling (pooling) layers. The use of convolutions has a two-fold effect. First, it allows extracting local features that are shared across the image domain and greatly reduces the number of parameters in the network with respect to generic deep architectures (and thus also the risk of overfitting), without sacrificing the expressive capacity of the network. Second, as we will show in the following, the convolutional architecture itself imposes some priors about the data, which appear very suitable especially for natural images \cite{goodfellow2013maxout,bruna2013invariant}. 


%Dealing with signals such as speech, images, or video on 1D-, 2D-, and 3D Euclidean domains, respectively, has been the main focus of research in deep learning for the past decades. 
%{\color{blue}
Deep learning models have been particularly successful when dealing with signals such as speech, images, or video, in which there is an underlying Euclidean structure. %}
% {\color{green} ADS: lots of work has focused on other things, it just hasn't been as successful.  not sure how to phrase... also, I think instead of ``on Euclidean domains'' vs. ``on Non-euclidean''  we should say ``on data with underlying Euclidean structure'' vs ``on data without underlying Euclidean structure''.  Although it is more wordy, it is less confusing...}
Recently, there has been a growing interest in trying to apply learning on non-Euclidean geometric data, for example in computer graphics and vision \cite{masci2015geodesic,boscaini2015learning,boscaini2016learning}, natural language processing \cite{bengio2003neural, mikolov2013efficient}, social network analysis \cite{perozzi2014deepwalk,tang2015line,cao2015grarep}, and biology \cite{alipanahi2015predicting,duvenaud2015convolutional}. 
The non-Euclidean nature of such data implies that there are no such familiar properties as global parameterization, common system of coordinates, vector space structure, or shift-invariance. Consequently, basic operations like linear combination or convolution that are taken for granted in the Euclidean case, are even not well defined on non-Euclidean domains. This happens to be a major obstacle that has so far precluded the use of successful deep learning methods such as convolutional networks on generic non-Euclidean geometric data. As a result, the quantitative and qualitative breakthrough that deep learning methods have brought into speech recognition, natural language processing, and computer vision has not yet come to fields dealing with geometric data. 



\section{Geometric learning problems}
\label{sec:problems}



Broadly speaking, we can distinguish between two classes of geometric learning problems.  
%%\paragraph*{\bf Building a domain} 
%
In the first class of problems, the goal is to characterize the {\em structure} of the data.  For example, given a set of data points with some underlying lower dimensional structure embedded into a high-dimensional Euclidean space, we may want to recover that lower dimensional structure.  This is often  referred to as {\em manifold learning}\footnote{Note that the notion of ``manifold'' in this setting can be  considerably more general than a classical smooth manifold; see e.g. \cite{non-differentiable_image,Verma:adaptive}}  or {\em non-linear dimensionality reduction}, and is an instance of unsupervised learning.  
%
Many methods for non-linear dimensionality reduction consist of two steps: first, they start with constructing a representation of local affinity of the data points (typically, a sparsely connected graph). Second, the data points are embedded into a low-dimensional space trying to preserve some criterion of the original affinity. For example, spectral embeddings tend to map points with many connections between them to nearby locations, and MDS-type methods try to preserve global information such as graph geodesic distances.   Examples of such methods include different flavors of multidimensional scaling (MDS) \cite{tenenbaum2000global}, locally linear embedding (LLE) \cite{roweis2000nonlinear}, stochastic neighbor embedding (t-SNE) \cite{maaten2008visualizing}, spectral embeddings such as Laplacian eigenmaps \cite{belkin2003laplacian} and diffusion maps \cite{coifman2006diffusion}, and deep models \cite{hadsell2006dimensionality,perozzi2014deepwalk,tang2015line,cao2015grarep}.    Instead of embedding the points, sometimes the graph can be processed directly, for example by decomposing it into small sub-graphs called {\em motifs} \cite{milo2002network} or  {\em graphlets} \cite{prvzulj2007biological}.  


In some cases, the data are presented as a manifold or graph at the outset, and the first step of constructing the affinity structure described above is unnecessary. 
% (at the cost of having to use the graph structure given, instead of the practitioner getting to choose it). 
For instance, in computer graphics and vision applications, one can analyze 3D shapes represented as meshes by constructing local geometric descriptors capturing e.g. curvature-like properties \cite{sun2009concise,litman2014learning}. 
%%
In network analysis applications such as computational sociology, the topological structure of the social graph  representing the social relations between people carries important insights allowing, for example, to classify the vertices and detect communities \cite{fortunato2010community}. 
%%
In natural language processing, words in a corpus can be represented by the co-occurrence graph, where two words are connected  if they often appear near each other \cite{mikolov2013distributed}.

  
%%
%Several recent approaches, notably DeepWalk \cite{perozzi2014deepwalk} and follow-up LINE \cite{tang2015line} and GraRep \cite{cao2015grarep} models, try to learn vertex-wise features that capture the local graph structure (or alternatively, embed the graph in a Euclidean space in a way that maps together vertices connected to their neighbors in a similar manner). 
%
%%
%These works essentially generalize the highly-successful {\em word2vec} learning paradigm \cite{mikolov2013distributed} developed in the natural language community to represent words in the Euclidean space in a context-preserving manner.  


%%
%Most of these methods consist of two ingredients: First, they start with constructing a representation of local affinity of the data points (typically, a sparsely connected graph). Second, the data points are embedded into a low-dimensional space trying to preserve the original affinity. For example, spectral embeddings tend to map points with many connections between them to nearby locations, and MDS-type methods try to preserve global information such as graph geodesic distances. 
%
%
%%\paragraph*{\bf Learning a domain} 
%The second class of problems deals with a given domain, and tries to characterize {\em the domain itself}. 
%%
%%For instance, in computer graphics and vision applications, many applications try to analyze 3D shapes represented as manifolds by constructing local geometric descriptors capturing e.g. curvature-like properties \cite{sun2009concise}. 
%%
%In network analysis applications such as computational sociology, the topological structure of the social graph  representing the social relations between people carries important insights allowing, for example, to classify the vertices and detect communities \cite{fortunato2010community}. 
%%
%Classical approaches analyze the graph by decomposing it into small sub-graphs called {\em motifs} \cite{milo2002network} or  {\em graphlets} \cite{prvzulj2007biological}.  
%%
%Several recent approaches, notably DeepWalk \cite{perozzi2014deepwalk} and follow-up LINE \cite{tang2015line} and GraRep \cite{cao2015grarep} models, try to learn vertex-wise features that capture the local graph structure (or alternatively, embed the graph in a Euclidean space in a way that maps together vertices connected to their neighbors in a similar manner). 
%
%%
%These works essentially generalize the highly-successful {\em word2vec} learning paradigm \cite{mikolov2013distributed} developed in the natural language community to represent words in the Euclidean space in a context-preserving manner.  




%
%
%%\paragraph*{\bf Building a domain} 
%In the first class of problems, we are given {\em only a set of data points} in some high-dimensional Euclidean space. In many cases, the data would form a low-dimensional non-linear subspace that can be modeled as a manifold, whose intrinsic dimensions relate to the `number of degrees of freedom' in the dataset. Reconstructing such a low-dimensional model from the data and using it to reason about the data is usually referred to as {\em manifold learning} or {\em non-linear dimensionality reduction}, and is an instance of unsupervised learning. {\color{green} ADS: Some note somewhere about what ``manifold'' should mean in this setting?  it isn't the classical manifolds discussed below.  Maybe a footnote?}
%%
%Classical examples of methods falling into this category include different flavors of multidimensional scaling (MDS) \cite{tenenbaum2000global}, locally linear embedding (LLE) \cite{roweis2000nonlinear}, stochastic neighbor embedding (t-SNE) \cite{maaten2008visualizing}, spectral embeddings such as Laplacian eigenmaps \cite{belkin2003laplacian} and diffusion maps \cite{coifman2006diffusion}, and deep models such as DrLIM \cite{hadsell2006dimensionality}. 
%%
%Most of these methods consist of two ingredients: First, they start with constructing a representation of local affinity of the data points (typically, a sparsely connected graph). Second, the data points are embedded into a low-dimensional space trying to preserve the original affinity. For example, spectral embeddings tend to map points with many connections between them to nearby locations, and MDS-type methods try to preserve global information such as graph geodesic distances. 
%
%
%%\paragraph*{\bf Learning a domain} 
%The second class of problems deals with a given domain, and tries to characterize {\em the domain itself}. 
%%
%%For instance, in computer graphics and vision applications, many applications try to analyze 3D shapes represented as manifolds by constructing local geometric descriptors capturing e.g. curvature-like properties \cite{sun2009concise}. 
%%
%In network analysis applications such as computational sociology, the topological structure of the social graph  representing the social relations between people carries important insights allowing, for example, to classify the vertices and detect communities \cite{fortunato2010community}. 
%%
%Classical approaches analyze the graph by decomposing it into small sub-graphs called {\em motifs} \cite{milo2002network} or  {\em graphlets} \cite{prvzulj2007biological}.  
%%
%Several recent approaches, notably DeepWalk \cite{perozzi2014deepwalk} and follow-up LINE \cite{tang2015line} and GraRep \cite{cao2015grarep} models, try to learn vertex-wise features that capture the local graph structure (or alternatively, embed the graph in a Euclidean space in a way that maps together vertices connected to their neighbors in a similar manner). 
%
%%
%These works essentially generalize the highly-successful {\em word2vec} learning paradigm \cite{mikolov2013distributed} developed in the natural language community to represent words in the Euclidean space in a context-preserving manner.  
%
%{\color{green} ADS: Is this really that different than the first class?  it seems to be the same thing, perhaps with the data given directly as a graph than as points in space to make a graph from.  In particular, deepwalk is just a matrix factorziation, and the only difference between the embeddings from deepwalk and say the embeddings from a Laplacian eigenmap embedding is whether you measure error in L2 or with a cross entropy loss}


%\paragraph*{\bf Learning on a domain} 
The second class of problems deals with analyzing {\em functions} defined on a given non-Euclidean domain (these two classes are related, since understanding the properties of functions defined on a domain conveys certain information about the domain, and vice-versa, the structure of the domain imposes certain properties on the functions on it).  
%
We can further break down such problems into two subclasses: problems where the domain is {\em fixed} and those where {\em multiple domains} are given. 
%
Resorting again to the social network example, assume that we are given the geographic coordinates of users at different time, represented as a time-dependent signal on the vertices of the graph. An important application in location-based social networks is to predict the position of the user given his or her past behavior, as well as that of his or her friends \cite{cho2011friendship}. 
%
In this problem, the domain (social graph) is assumed to be fixed; methods of {\em signal processing on graphs}, which have previously been reviewed in Signal Processing Magazine \cite{shuman2013emerging}), can be applied to this setting, in particular, in order to define an operation similar to convolution in the spectral domain. This, in turn, allows generalizing  CNN models to graphs \cite{henaff2015deep,defferrard2016convolutional}. 
%

In computer graphics and vision applications, finding similarity and correspondence between shapes are examples of the second sub-class of problems: each shape is modeled as a manifold, and one has to work with multiple such domains. 
%
In this setting, a generalization of convolution in the spatial domain using local charting  \cite{atwood2016search,masci2015geodesic,boscaini2016learning} appears to be more appropriate. 


%In computer graphics applications, a generalization of CNNs working on local intrinsic local patches was applied on 3D deformable shapes modeled as manifolds to address problems such as correspondence and similarity \cite{masci2015geodesic,boscaini2016learning}.



The main focus of this review is on the this second class of problems, namely learning functions non-Euclidean structured domains, and in particular, attempts to generalize the popular CNNs to such settings. 
%
%We will consider both single- and multiple-domain cases. 
%
We will start with an overview of Euclidean deep learning, summarizing the important assumptions about the data, and how they are realized in convolutional network architectures. 
%
For a more in-depth review of CNNs and their and applications, we refer the reader to \cite{lecun2015deep} and references therein.


Going to the non-Euclidean world, we will then define basic notions in differential geometry and graph theory. These topics are insufficiently known in the signal processing community, and to our knowledge, there is no introductory-level reference treating these so different structures in a common way. One of our goals in this review is to provide an accessible overview of these models resorting as much as possible to the intuition of traditional signal processing. 
%
We will emphasize the similarities and the differences between Euclidean and non-Euclidean domains, and distinguish between spatial- and spectral domain learning methods. 
%We will further distinguish between methods that assume the domain to be fixed and those that can adapt to different domains. 


Finally, we will show examples of selected problem from the fields of network analysis, computer vision, and graphics, and outline current main challenges and potential future research directions.   


%In the next sections, we will start with reviewing the basic ideas of classical deep learning on Euclidean domains (images) and then see the differences and challenges introduced by the need to deal with a non-Euclidean domains. 
% 
%
%
\myframedtext[0.95\linewidth]{
%
%\paragraph*{\bf Notation}\\
\begin{tabular}{ l l }
{\bf Notation} &\\
  $\mathbb{R}^m$ & $m$-dimensional Euclidean space\\
  $a, \mathbf{a}, \mathbf{A}$ & Scalar, vector, matrix\\
  $\Omega, x$ & Arbitrary domain, coordinate on it \\
  $f\in L^2(\Omega)$ & Square-integrable function on $\Omega$ \\
  $\mathcal{T}_v$ & Translation operator\\
  $\tau, \mathcal{L}_\tau$ & Deformation field, operator\\
  $\hat{f}$ & Fourier transform of $f$ \\
  $f \star g$ & Convolution of $f$ and $g$ \\
  $\mathcal{X}, T\mathcal{X}, T_x \mathcal{X}$ & Manifold, its tangent bundle, tangent \\ & space at $x$\\  
  $\langle \cdot, \cdot, \rangle_{T\mathcal{X}}$ & Riemannian metric \\  
  $f\in L^2(\mathcal{X})$ & Scalar field on manifold $\mathcal{X}$ \\  
  $F\in L^2(T\mathcal{X})$ & Tangent vector field on manifold $\mathcal{X}$ \\  
  $\nabla, \mathrm{div}, \Delta$ & Gradient, divergence, Laplace operators \\  
  $\mathcal{V}, \mathcal{E}, \mathcal{F}$ & Vertices and edges of a graph, \\  
  & faces of a mesh \\  
  %
  $f\in L^2(\mathcal{V})$ & Functions on vertices of a graph\\  
  $F\in L^2(\mathcal{E})$ & Functions on edges of a graph \\  
  %  
  $\phi_i, \lambda_i$ & Laplacian eigenfunctions, eigenvalues \\  
  $h_t(\cdot, \cdot)$ & Heat kernel \\  
  %
  $\boldsymbol{\Phi}_k$ & Matrix of first $k$ Laplacian eigenvectors \\  
  $\boldsymbol{\Lambda}_k$ & Diagonal matrix of first $k$ Laplacian  \\  
  & eigenvalues\\
  %
  $\xi$ & point-wise nonlinearity \\
  $w_{l,l'}(x), \mathbf{W}_{l,l'}$ & Convolutional filter in spatial\\& and spectral domain\\
  %
\end{tabular}
%
%We denote by $\Omega$ an arbitrary domain, by $x \in \Omega$ a coordinate in this domain, 
%and by $f(x)$ a function or image defined on that domain. 
%$f \in L^2(\Omega, \R^m)$ if $f(x) \in \R^m$ and
%it is square integrable: $\|f \|_2^2= \int \|f(x)\|^2 dx < \infty$, 
%and $f \in L^1(\Omega,\R^m)$ if it is absolutely integrable: $\|f \|_1 = \int |f(x)| dx < \infty$.
%For simplicity, we write $L^p(\Omega) = L^p(\Omega, \R)$.
%The Fourier transform of $f \in L^2(\Omega, \R)$ is denoted as 
%$\hat{f}(\omega) = \int f(x) e^{-i x.\omega } dx$.
%Given $f, g \in L^1(\Omega)$, the convolution is 
%$f \star g(x) = \int f(x') g(x-x') dx'$.
%Matrices are denoted in bold-face $\mathbf{X}$.
%[Introduce here the notation concerning the Graph Laplacian].
%
}








%At this point, we should introduce a more precise terminology, which we will define in the next sections. 
%By non-Euclidean domains, we refer to two prototypical structures: graphs and manifolds. The latter, being a continuous structure, can be discretized in many ways, also as a graph. The main characteristic of a manifold when compared to 


